What Have We Achieved on Non-autoregressive Translation?

Recent advances have made non-autoregressive (NAT) translation comparable to autoregressive methods (AT). However, their evaluation using BLEU has been shown to weakly correlate with human annotations. Limited research compares non-autoregressive translation and autoregressive translation comprehensively, leaving uncertainty about the true proximity of NAT to AT. To address this gap, we systematically evaluate four representative NAT methods across various dimensions, including human evaluation. Our empirical results demonstrate that despite narrowing the performance gap, state-of-the-art NAT still underperforms AT under more reliable evaluation metrics. Furthermore, we discover that explicitly modeling dependencies is crucial for generating natural language and generalizing to out-of-distribution sequences.

==> table/hallucination.tex <==
% \begin{table*}[t]
% \centering
% % \small
% % \setlength{\tabcolsep}{1.1pt}
% % \def\arraystretch{1.5}
% \begin{tabular}{lcccc}
% \thickhline
% Models  & \multicolumn{1}{l}{xnli} & \multicolumn{1}{l}{LaBse} & \multicolumn{1}{l}{qe-based} & \multicolumn{1}{l}{qe-free}  \\
% \hline
% % big    &30.82 & 32.25   & - & -    & - & -   & -    \\
% base   & 0.989  & 0.905   & 0.0070     & 0.0464    \\
% base-kd & 0.983 & 0.905   & 0.0140     & 0.0497     \\
% vanilla NAT  & 0.949 & 0.742   & -0.3340     & -0.2403     \\
% vanilla NAT kd    &0.975     & 0.87   & -0.0914	 &-0.0418   \\
% CTC & 0.977&	0.876&	-0.0913&	-0.0353  \\
% CTC kd   & 0.986&	0.896& 	-0.0397 &	0.0025    \\
% CMLM(K=10) & 0.966&	0.844&	-0.0914&	-0.0253  \\
% CMLM(K-10)KD  & 0.965&	0.841&	-0.0835&	-0.0198 \\
% MGMO  &0.985&	0.887&	-0.0683&	-0.0193   \\
% MGMO kd  & 0.986&	0.888&	-0.0298&	-0.0170	  \\
% DA   & 0.989&	0.89	&-0.0268&	0.0154   \\
% DA-kd   & 0.991&	0.901&	-0.0014&	0.0347  \\

% \thickhline
% \label{tab:main}
% \end{tabular}
% \caption{Hallucination
% }
% \end{table*}

\begin{table}[t]
\centering
\small
% \setlength{\tabcolsep}{1.1pt}
% \def\arraystretch{1.5}
\begin{tabular}{lcc}
\thickhline
Models  & \multicolumn{1}{l}{xnli} & \multicolumn{1}{l}{LaBse}  \\
\hline
base   & 0.99  & 0.91   \\
vanilla NAT  & 0.949 & 0.742    \\
CTC & 0.977&	0.876 \\
CMLM & 0.966&	0.844 \\
MGMO  &0.985&	0.887 \\
DA   & 0.989&	0.89	 \\

\thickhline
\label{tab:main}
\end{tabular}
\caption{Hallucination
}
\end{table}

==> table/main.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.05} 
% \setlength{\tabcolsep}{1.1pt}
% \def\arraystretch{1.5}
\begin{tabular}{lcccccc}
\toprule
Model  & \multicolumn{1}{l}{BLEU$\uparrow$}&\multicolumn{1}{l}{chrf$\uparrow$} & \multicolumn{1}{l}{COMET$\uparrow$}&\multicolumn{1}{l}{BLEURT$\uparrow$} &\multicolumn{1}{l}{GEMBA$\uparrow$} &\multicolumn{1}{l}{Speed$\uparrow$}\\
\midrule
% big    &30.82 & 32.25&&& &  \\
\multicolumn{7}{c}{w/o Knowledge Distillation} \\
\midrule
AT~\cite{VaswaniSPUJGKP17} & \textbf{31.89} & \textbf{60.25} &\textbf{84.26$\dagger$}&\textbf{71.94$\dagger$}& \textbf{92.91$\dagger$}  & \\
NAT~\cite{nat}  & 16.85 & 43.46   &55.87&44.80&36.94  &\\
MgMO~\cite{mgmo} & 28.89&58.11 & 77.76&64.08&83.51  &\\
CTC~\cite{ctc}  & 27.35 &56.53 & 75.38& 61.79&79.14  & \\
DAT~\cite{da}  & 31.69 &59.60 &81.12&69.00&88.29  & \\
CMLM~\cite{maskp} & 29.36 & 57.79 &76.39&65.00&82.07  &\\
% DA ()   & 29.83 & 31.69    \\
\midrule
\multicolumn{7}{c}{w/ Knowledge Distillation} \\
\midrule
AT~\cite{VaswaniSPUJGKP17}  & 32.04 &\textbf{60.85}&\textbf{84.72$\dagger$}& \textbf{72.53} &  \textbf{93.39$\dagger$} & \\
NAT~\cite{nat}  &27.55&56.56 &75.50&62.72&76.89 & \\
MgMO~\cite{mgmo}  & 30.32&59.36 &81.15&67.76 &89.17  &\\
CTC~\cite{ctc}    & 30.52&59.83   &80.06&67.24& 86.91  &\\
DAT~\cite{da}   &\textbf{32.26}&60.80 &83.32&71.44& 92.05  & \\
CMLM~\cite{maskp} & 30.25& 58.40 &77.14&65.63& 82.98  &\\
\bottomrule
\label{tab:main}
\end{tabular}
\caption{
Automatic evaluation results of different translation models on WMT21 De$\Rightarrow$En, considering both raw data and distillation data settings.
We encompass a wide range of metrics including rule-based metrics (BLEU and chrf), model-based metrics (COMET and BLEURT) and LLM-based metrics (GEMBA).
Bold numbers represent the best performance.
$\dagger$ denotes translation quality of AT is significantly better than all other models with a $p<0.01$ \cite{sigtest}.
% $\dagger$ denotes translation quality is significantly lower than that of the AT counterpart with a $p<0.01$ \cite{sigtest}.
}
\end{table*}


% \begin{table*}[t]
% \centering
% \small
% \renewcommand{\arraystretch}{1.1} 
% % \setlength{\tabcolsep}{1.1pt}
% % \def\arraystretch{1.5}
% \begin{tabular}{lccccccc}
% \toprule
% Models & \multicolumn{1}{l}{greedy} & \multicolumn{1}{l}{beam} & \multicolumn{1}{l}{comet}&\multicolumn{1}{l}{BLEURT} &\multicolumn{1}{l}{chrf}&\multicolumn{1}{l}{GPT4-Eval}\\
% \midrule
% % big    &30.82 & 32.25&&& &  \\
% AT~\cite{VaswaniSPUJGKP17} & 30.56 & 31.89 &&71.94&60.2& 92.912  \\
% w/ KD & 31.85 & 32.04 && 72.53&60.8 &  93.387 \\
% vanilla NAT~\cite{nat} &16.00 & 16.85   &&44.80&43.5 &36.938\\
% w/ KD  & 25.35  &27.55 &&62.72&56.6&76.886 \\
% CTC~\cite{ctc} &27.55 & 27.35 && 61.79&56.5 &79.136   \\
% w/ KD   & 30.50& 30.52 &&67.24&59.8  & 86.914\\
% CMLM~\cite{maskp} & 29.10 & 29.36 &&65.00& 57.8 &82.067\\
% w/ KD   &30.37 & 30.25 &&65.63& 58.4& 82.982\\
% MGMO~\cite{mgmo} &28.36& 28.89 &&64.08&58.1&83.508  \\
% w/ KD   & 30.05 & 30.32 &&67.76&59.4 &89.174\\
% DA~\cite{da}   & 29.83 & 31.69 &&&59.6&88.285   \\
% % DA ()   & 29.83 & 31.69    \\
% w/ KD   &31.53 &32.26 &&71.44&60.8& 92.046 \\

% \bottomrule
% \label{tab:main}
% \end{tabular}
% \caption{main table
% }
% \end{table*}

==> table/main_enro.tex <==
\begin{table*}[t]
\centering
\small
\renewcommand{\arraystretch}{1.05} 
% \setlength{\tabcolsep}{1.1pt}
% \def\arraystretch{1.5}
\begin{tabular}{lcccccc}
\toprule
Model  & \multicolumn{1}{l}{BLEU$\uparrow$}&\multicolumn{1}{l}{chrf$\uparrow$} & \multicolumn{1}{l}{COMET$\uparrow$}&\multicolumn{1}{l}{BLEURT$\uparrow$} &\multicolumn{1}{l}{GEMBA$\uparrow$} &\multicolumn{1}{l}{Speed$\uparrow$}\\
\midrule
% big    &30.82 & 32.25&&& &  \\


\multicolumn{7}{c}{w/o Knowledge Distillation} \\
\midrule
AT~\cite{VaswaniSPUJGKP17} & 34.39 & 58.48 & 78.90 &69.89  & &\\
NAT~\cite{nat}   &  &  &  &  & &\\
MgMO~\cite{mgmo}  &  30.97 & 56.65 & 73.54 & 63.19 & &\\
CTC~\cite{ctc}  &32.73  & 57.77 & 74.26 &  63.99& &\\
DAT~\cite{da}  & 33.18 & 57.35 &76.14  &  66.72& &\\
CMLM~\cite{maskp}  & 31.97 & 56.78 & 74.11 & 63.34 & &\\
% DA ()   & 29.83 & 31.69    \\
\midrule

\multicolumn{7}{c}{w/ Knowledge Distillation} \\
\midrule
AT~\cite{VaswaniSPUJGKP17}   &33.92  & 58.45 &  78.49& 69.26 & &\\
NAT~\cite{nat}   & 30.97 & 56.52 & 72.60 & 62.12 & &\\
MgMO~\cite{mgmo} & 32.86 & 57.40 & 75.52 &65.36  & &\\ 
CTC~\cite{ctc}    &  &  &  &  & &\\
DAT~\cite{da}   &  33.25 & 57.89 & 76.59 & 67.01 & &\\
CMLM~\cite{maskp} & 32.71 & 56.76 & 72.36 & 63.42 & &\\
\bottomrule
\label{tab:main_enro}
\end{tabular}
\caption{
Automatic evaluation results of different translation models on WMT14 En$\Rightarrow$Ro, considering both raw data and distillation data settings.
We encompass a wide range of metrics including rule-based metrics (BLEU and chrf), model-based metrics (COMET and BLEURT) and LLM-based metrics (GEMBA).
Bold numbers represent the best performance.
$\dagger$ denotes translation quality of AT is significantly better than all other models with a $p<0.01$ \cite{sigtest}.
% $\dagger$ denotes translation quality is significantly lower than that of the AT counterpart with a $p<0.01$ \cite{sigtest}.
}
\end{table*}

